Expository Text Generation: Imitate, Retrieve, Paraphrase

Expository documents are vital resources for conveying complex information to readers. Despite their usefulness, writing expository text by hand is a challenging process that requires careful content planning, obtaining facts from multiple sources, and the ability to clearly synthesize these facts. To ease these burdens, we propose the task of expository text generation, which seeks to automatically generate an accurate and stylistically consistent expository text for a topic by intelligently searching a knowledge source. We solve our task by developing IRP, a framework that overcomes the limitations of retrieval-augmented models and iteratively performs content planning, fact retrieval, and rephrasing. Through experiments on three diverse, newly-collected datasets, we show that IRP produces factual and organized expository texts that accurately inform readers.

==> data/component.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{\label{table:component} Performance comparison of Imitator (median perplexity), Retriever (classification accuracy), and Paraphraser (METEOR \emph{with doc}\textbf{/}\emph{without doc}) per test set.}
\begin{tabular}{@{}l|c|c|c@{}}
\toprule
\textbf{Component}  & \textbf{U.S. News} & \textbf{Medline} & \textbf{WikiCS} \\ \midrule
Imitator - \textit{Perplexity} & 16.43              & 70.01            & 31.03           \\
Retriever - \textit{Accuracy}  & 0.966              & 0.622            & 0.416           \\
Paraphraser - \textit{METEOR}  & 0.66/0.62          & 0.52/0.44        & 0.35/0.14              \\ \bottomrule
\end{tabular}
\end{table}

==> data/corr.tex <==
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{2pt}
\caption{\label{table:corr} Spearman's correlation coefficient between human evaluation and \emph{factuality metrics}. Darker shades of \colorbox{blue!20}{blue} and \colorbox{red!20}{red} indicate stronger positive and negative correlations with human evaluations, respectively. \jie{delete or move to Appendix?}}
\vspace{-1.5ex}
\begin{tabular}{@{}c|c|c|c|c@{}}
\toprule
\textbf{Dataset}               & \textbf{Halluc} & \textbf{FactCC} & \textbf{NLI-Ent} & \textbf{NLI-Contr} \\ \midrule
U.S. News \emph{with doc}    & \cellcolor{color1}-0.36  & \cellcolor{color2}-0.17  & \cellcolor{color3}0.41    & \cellcolor{color4}0.01      \\
U.S. News \emph{w/out doc} & \cellcolor{color5}-0.11  & \cellcolor{color6}0.27   & \cellcolor{color7}0.21    & \cellcolor{color8}-0.28     \\
Medline \emph{with doc}      & \cellcolor{color9}0.18   & \cellcolor{color10}-0.49  & \cellcolor{color11}0.01    & \cellcolor{color12}-0.04     \\
Medline \emph{w/out doc}   & \cellcolor{color13}-0.09  & \cellcolor{color14}0.03   & \cellcolor{color15}0.43    & \cellcolor{color16}-0.07     \\ \bottomrule
\end{tabular}
\vspace{-3.2ex}
\end{table}

==> data/human_full.tex <==
\begin{table}[t]
\small
\setlength{\tabcolsep}{3pt}
\caption{\label{table:human} Human evaluation of model outputs on grammaticality, informativeness, and factual accuracy.}
\begin{tabular}{@{}clcccccc@{}}
\multicolumn{1}{l}{} &  & \multicolumn{3}{c}{\textit{w/ doc}} & \multicolumn{3}{c}{\textit{w/out doc}} \\ \midrule
\multicolumn{1}{l|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Gram} & \textbf{Inf} & \multicolumn{1}{c|}{\textbf{Fact}} & \textbf{Gram} & \textbf{Inf} & \textbf{Fact} \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}U.S. \\ News\end{tabular}}} & \multicolumn{1}{l|}{IRP} & 4.95 & 5.00 & \multicolumn{1}{c|}{\textbf{4.63}} & 4.95 & 4.89 & \textbf{3.78} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{LED} & 4.90 & 4.78 & \multicolumn{1}{c|}{2.03} & 4.95 & 4.89 & 2.18 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{RAG} & 5.00 & 5.00 & \multicolumn{1}{c|}{2.60} & 4.98 & 4.98 & 2.90 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{BART} & 5.00 & 5.00 & \multicolumn{1}{c|}{1.80} & 4.98 & 4.90 & 1.73 \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Medline}} & \multicolumn{1}{l|}{IRP} & 4.73 & 4.78 & \multicolumn{1}{c|}{1} & 1 & 1 & 1 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{LED} & 4.1 & 3.33 & \multicolumn{1}{c|}{1} & 1 & 1 & 1 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{RAG} & 4.80 & 4.10 & \multicolumn{1}{c|}{1} & 1 & 1 & 1 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{BART} & 5.00 & 1.5 & \multicolumn{1}{c|}{1} & 1 & 1 & 1 \\ \bottomrule
\end{tabular}
\end{table}

==> data/performance_leak.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}clcccccccc@{}}
\textbf{} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{4}{c}{\textit{Traditional Metrics}} & \multicolumn{4}{c}{\textit{Faithfulness Metrics}} \\ \midrule
\multicolumn{1}{c|}{\textbf{Datasets}} & \multicolumn{1}{c|}{\textbf{Models}} & \textbf{R1} & \textbf{R2} & \textbf{BLEU} & \multicolumn{1}{c|}{\textbf{METEOR}} & \textbf{Halluc.} & \textbf{FactCC} & \textbf{MNLI-Ent} & \textbf{MNLI-Con} \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{College}} & \multicolumn{1}{l|}{Ours} & \textbf{0.894} & \textbf{0.787} & \textbf{0.759} & \multicolumn{1}{c|}{\textbf{0.882}} & \textbf{2.65} & \textbf{0.851} & \textbf{0.878} & \textbf{0.035} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{Longformer} & 0.754 & 0.612 & 0.577 & \multicolumn{1}{c|}{0.784} & 6.04 & 0.476 & 0.395 & 0.458 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{RAG} & 0.783 & 0.641 & 0.603 & \multicolumn{1}{c|}{0.809} & 5.97 & 0.481 & 0.415 & 0.532 \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{Medicine}} & \multicolumn{1}{l|}{Ours} & 0.594 & \textbf{0.490} & \textbf{0.406} & \multicolumn{1}{c|}{\textbf{0.529}} & \textbf{1.18} & \textbf{0.918} & \textbf{0.526} & \textbf{0.140} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{Longformer} & 0.491 & 0.300 & 0.210 & \multicolumn{1}{c|}{0.404} & 2.16 & 0.859 & 0.322 & 0.282 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{RAG} & \textbf{0.596} & 0.449 & 0.384 & \multicolumn{1}{c|}{\textbf{0.529}} & 2.36 & 0.873 & 0.423 & 0.221 \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{Wikipedia}} & \multicolumn{1}{l|}{Ours} & \textbf{0.435} & \textbf{0.341} & \textbf{0.216} & \multicolumn{1}{c|}{\textbf{0.354}} & 0.84 & \textbf{0.658} & \textbf{0.516} & \textbf{0.147} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{Longformer} & 0.253 & 0.084 & 0.037 & \multicolumn{1}{c|}{0.163} & \textbf{0.83} & 0.329 & 0.162 & 0.220 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{RAG} & 0.333 & 0.159 & 0.142 & \multicolumn{1}{c|}{0.278} & 3.14 & 0.546 & 0.194 & 0.18 \\ \bottomrule
\end{tabular}
\end{table*}

==> data/performance_no_leak.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}c|l|cccc|cccc@{}}
\toprule
\textbf{Datasets} & \multicolumn{1}{c|}{\textbf{Models}} & \textbf{R1} & \textbf{R2} & \textbf{BLEU} & \textbf{METEOR} & \textbf{Halluc.} & \textbf{FactCC} & \textbf{MNLI-Ent} & \textbf{MNLI-Con} \\ \midrule
\multirow{3}{*}{College} & Ours & 0.706 & 0.496 & 0.453 & 0.703 & \textbf{2.86} & \textbf{0.227} & \textbf{0.514} & \textbf{0.410} \\
 & \multicolumn{1}{c|}{Longformer} & 0.744 & 0.594 & \textbf{0.696} & 0.784 & 6.69 & 0.217 & 0.334 & 0.544 \\
 & RAG & \textbf{0.787} & \textbf{0.602} & 0.632 & \textbf{0.817} & 6.20 & 0.202 & 0.363 & 0.591 \\ \midrule
\multirow{3}{*}{Medicine} & Ours & 0.526 & \textbf{0.364} & 0.275 & 0.445 & \textbf{1.31} & \textbf{0.854} & \textbf{0.475} & \textbf{0.187} \\
 & Longformer & 0.478 & 0.284 & 0.194 & 0.391 & 1.92 & 0.838 & 0.341 & 0.251 \\
 & RAG & \textbf{0.527} & 0.343 & \textbf{0.281} & \textbf{0.462} & 2.83 & 0.812 & 0.339 & 0.194 \\ \midrule

 \multirow{3}{*}{Wikipedia} & Ours & 0.526 & \textbf{0.364} & 0.275 & 0.445 & \textbf{1.31} & \textbf{0.854} & \textbf{0.475} & \textbf{0.187} \\
 & Longformer & 0.478 & 0.284 & 0.194 & 0.391 & 1.92 & 0.838 & 0.341 & 0.251 \\
 & RAG & \textbf{0.527} & 0.343 & \textbf{0.281} & \textbf{0.462} & 2.83 & 0.812 & 0.339 & 0.194 \\ \bottomrule
\end{tabular}
\end{table*}
